The MATLAB Toolbox SciXMiner: User's Manual and Programmer's Guide

The Matlab toolbox SciXMiner is designed for the visualization and analysis of time series and features with a special focus to classification problems. It was developed at the Institute of Applied Computer Science of the Karlsruhe Institute of Technology (KIT), a member of the Helmholtz Association of German Research Centres in Germany. The aim was to provide an open platform for the development and improvement of data mining methods and its applications to various medical and technical problems. SciXMiner bases on Matlab (tested for the version 2017a). Many functions do not require additional standard toolboxes but some parts of Signal, Statistics and Wavelet toolboxes are used for special cases. The decision to a Matlab-based solution was made to use the wide mathematical functionality of this package provided by The Mathworks Inc. SciXMiner is controlled by a graphical user interface (GUI) with menu items and control elements like popup lists, checkboxes and edit elements. This makes it easier to work with SciXMiner for inexperienced users. Furthermore, an automatization and batch standardization of analyzes is possible using macros. The standard Matlab style using the command line is also available. SciXMiner is an open source software. The download page is http://sourceforge.net/projects/SciXMiner. It is licensed under the conditions of the GNU General Public License (GNU-GPL) of The Free Software Foundation.

==> mydef.tex <==
\newenvironment{aufz}{
%\renewcommand{\labelitemi}{-}
\vspace{-1ex plus.25ex minus.25ex}\begin{itemize}\topsep0pt\itemsep0pt
\partopsep0pt}{\end{itemize}\vspace{-1ex plus0.25ex  minus.25ex}}


\newenvironment{numer}{
\renewcommand{\labelenumi}{(\itshape\roman{enumi})}
\renewcommand{\labelenumii}{(\itshape\alph{enumii})}
\vspace{-1ex plus.25ex minus.25ex}\begin{enumerate}\topsep0pt\itemsep0pt
\partopsep0pt}{\end{enumerate}\vspace{-1ex plus0.25ex minus.25ex}}

\newenvironment{numer2}{
\renewcommand{\labelenumi}{\arabic{enumi}.}
\renewcommand{\labelenumii}{(\alph{enumii})}
\vspace{-1ex plus.25ex minus.25ex}\begin{enumerate}\topsep0pt\itemsep0pt
\partopsep0pt}{\end{enumerate}\vspace{-1ex plus0.25ex minus.25ex}}

%\newenvironment{textaufz}{\begin{list}{-}{\topsep0pt\parskip0pt\partopsep0pt
%\itemsep0pt\parsep0pt}}{\end{list}}

\newenvironment{textaufz}{\begin{list}{-}{
\setlength{\topsep}{0ex plus0.0ex minus0.0ex}
\setlength{\parskip}{0ex}
\setlength{\partopsep}{0ex}
\setlength{\itemsep}{0pt}
\setlength{\parsep}{0pt}
}}{\end{list}\vspace{-1.45ex}}%-0.25\baselineskip}}

% modif. Anordnung von figures
\setcounter{totalnumber}{8}
\setcounter{bottomnumber}{6}
\setcounter{topnumber}{6}

\renewcommand{\topfraction}{0.99}
\renewcommand{\bottomfraction}{0.99}
\renewcommand{\textfraction}{0.01}
\renewcommand{\floatpagefraction}{0.701}
% Ende

% Definition eigener Befehle
\newcommand{\bm}[1]{\mbox{\boldmath{$#1$}}}
\newcommand{\bmss}[1]{\mbox{\tiny\boldmath{$#1$}}}
\newcommand{\bms}[1]{\mbox{\scriptsize\boldmath{$#1$}}}
\newcommand{\bsym}[1]{\boldsymbol{#1}}
\newcommand{\D}{\displaystyle}
\newcommand{\T}{\textstyle}
\newcommand{\Sst}{\scriptstyle}
%\newcommand{\SS}{\scriptscriptstyle}
\newcommand{\gldef}{\stackrel{\rm def}{=}}
%\newcommand{\glnat}{\stackrel{=}{\rm\scriptstyle nat}}
\newcommand{\glnat}{\begin{array}[t]{@{\,}c@{\,}}
        =\\[-2ex] {\rm\scriptstyle nat}\end{array}}
%\newcommand{\gnat}{\stackrel{>}{\rm\scriptstyle nat}}
\newcommand{\gnat}{\begin{array}[t]{@{\,}c@{\,}}
        >\\[-2ex] {\rm\scriptstyle nat}\end{array}}
%\newcommand{\genat}{\stackrel{\geq}{\rm\s nat}}
\newcommand{\genat}{\begin{array}[t]{@{\,}c@{\,}}
        \ge\\[-1.3ex] {\rm\scriptstyle nat}\end{array}}
%\newcommand{\lnat}{\stackrel{<}{\rm\scriptstyle nat}}
\newcommand{\lnat}{\begin{array}[t]{@{\,}c@{\,}}
        <\\[-2ex] {\rm\scriptstyle nat}\end{array}}
%\newcommand{\lenat}{\stackrel{\leq}{\rm\scriptstyle nat}}
\newcommand{\lenat}{\begin{array}[t]{@{\,}c@{\,}}
        \le\\[-1.8ex] {\rm\scriptstyle nat}\end{array}}
\newcommand{\entspr}{\stackrel{\triangle}{=}}
% end Def. eigener Befehle

